Gotta Catch 'em All: Aggregating CVSS Scores

Security metrics are not standardized, but inter-national proposals such as the Common Vulnerability ScoringSystem (CVSS) for quantifying the severity of known vulnerabil-ities are widely used. Many CVSS aggregation mechanisms havebeen proposed in the literature. Nevertheless, factors related tothe context of the System Under Test (SUT) are not taken intoaccount in the aggregation process; vulnerabilities that in theoryaffect the SUT, but are not exploitable in reality. We propose aCVSS aggregation algorithm that integrates information aboutthe functionality disruption of the SUT, exploitation difficulty,existence of exploits, and the context where the SUT operates.The aggregation algorithm was applied to OpenPLC V3, showingthat it is capable of filtering out vulnerabilities that cannot beexploited in the real conditions of deployment of the particularsystem. Finally, because of the nature of the proposed algorithm,the result can be interpreted in the same way as a normal CVSS.

==> docs/Background.tex <==
% =================================================================================
% === II. BACKGROUND ==============================================================
% =================================================================================
\section{Background}
   


==> docs/Use_Case.tex <==
% =================================================================================
% === V. USE CASE =================================================================
% =================================================================================
\section{Use Case}
\label{sec:useCase}
    To test the potential of our proposal, we generated five different datasets of CVSSs, to test five different scenarios. For each one, we assigned random values of the correction factors. Finally, we obtained the aggregated value for each dataset using the proposed algorithm.

    
    \subsection{Initial dataset}
        To test our approach, we generated five datasets, each one containing 64 different CVSS values. Figure~\ref{fig:setOfDistributions} shows the CVSS distribution for each set:

        \begin{enumerate}
            \item \textbf{Distribution \#1:} The majority of the CVSS values in this dataset are concentrated around 5, and therefore, its mean would be also a value near 5.
            \item \textbf{Distribution \#2:} Most of the values of this dataset tend to be around high values of the scale.
            \item \textbf{Distribution \#3:} This dataset has the majority of its values around the low end of the scale.
            \item \textbf{Distribution \#4:} This dataset distributes its values on the ends of the scale (high and low values), letting values around five uncovered.
            \item \textbf{Distribution \#5:} This dataset represents a system whose CVSS values are equally distributed.
        \end{enumerate}
        
        With these datasets, we aim to cover the most common scenarios that can be faced when aggregating CVSS values in any given SUT.

        \begin{figure*}[!htb]
            \centering
            \begin{subfigure}{0.185\textwidth}
                \includegraphics[width=\textwidth]{photo/distribution_1.jpg}
                \caption{\centering$\bar{x}_1 = 5.11$\newline \centerline{$ba_1 = 8.04$}}
                \label{fig:firstDistribution}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.185\textwidth}
                \includegraphics[width=\textwidth]{photo/distribution_2.jpg}
                \caption{\centering$\bar{x}_2 = 7.09$\newline \centerline{$ba_2 = 8.59$}}
                \label{fig:secondDistribution}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.185\textwidth}
                \includegraphics[width=\textwidth]{photo/distribution_3.jpg}
                \caption[justification=centering]{\centering$\bar{x}_3 = 2.79$\newline \centerline{$ba_3 = 6.42$}}
                \label{fig:thirdDistribution}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.185\textwidth}
                \includegraphics[width=\textwidth]{photo/distribution_4.jpg}
                \caption{\centering$\bar{x}_4 = 5.14$\newline \centerline{$ba_4 = 8.05$}}
                \label{fig:fourthDistribution}
            \end{subfigure}
            \hfill
            \begin{subfigure}{0.185\textwidth}
                \includegraphics[width=\textwidth]{photo/distribution_5.jpg}
                \caption{\centering$\bar{x}_5 = 5.36$\newline \centerline{$ba_5 = 8.14$}}
                \label{fig:fithDistribution}
            \end{subfigure}
            \caption{The five CVSS distribution generated to test the aggregation algorithm. Each one represents a different scenario to test the proposed aggregation algorithm. $\bar{x}$ represents the arithmetic mean of all the values, and $ab$, the result of the Bayesian addition proposed in this research work.}
            \label{fig:setOfDistributions}
        \end{figure*}

    \subsection{Generation of the Correction Factors}
        In this stage, we compute the correcting factors for each CVSS, for each dataset. Correcting factors were generated randomly in the following sequence:
        
        \begin{enumerate}
            \item \textbf{Maximum distance from the entry point:} First, a number between $[2 , 20]$ was randomly picked to be the deepest level of dependency between the assets in the SUT.
    
            \item \textbf{Distance from the entry point:} Then, for each CVSS, we assigned a random value between 1 and the previously chosen maximum distance, to indicate in which location the CVSS is.
    
            \item \textbf{Deepness factor:} With the previous information, the deepness factor was calculated. For this, we supposed an equal distribution of the factor. Therefore, a linear interpolation was used.
    
            \item \textbf{Functionality factor:} Then, we generated the functionality factor, as a random binary number. A ``$0$'' indicates that functionality is not affected, whereas a ``$1$''indicates that functionality is affected by the given CVSS.
            
            \item \textbf{Context factor:} A randomly generated binary value $[0, 1]$ indicates whether the vulnerability associated to a CVSS is exploitable in the context of the SUT.
            
            \item \textbf{Exploit factor:} For each CVSS, a random value $\left\{0, 1.25, 1.5, 1.75, 2\right\}$ was chosen to indicate whether an exploit for that vulnerability exists, and to describe its development status.
            
            \item \textbf{Summarized correction factor:} Now, its possible to obtain the final correction factor for each CVSS by multiplying all the above calculated correction factors.
        \end{enumerate}
    
    
        % \begin{figure}[!htb]
        %     \centering
        %     \begin{subfigure}{0.2\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_1.jpg}
        %         \caption{$\bar{x}_1 = 5.11, ba_1 = 8.04$.}
        %         \label{fig:firstDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.2\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_2.jpg}
        %         \caption{$\bar{x}_2 = 7.09, ba_2 = 8.59$.}
        %         \label{fig:secondDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \vskip\baselineskip
        %     \begin{subfigure}{0.2\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_3.jpg}
        %         \caption{$\bar{x}_3 = 2.79, ba_3 = 6.42$.}
        %         \label{fig:thirdDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.2\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_4.jpg}
        %         \caption{$\bar{x}_4 = 5.14, ba_4 = 8.05$.}
        %         \label{fig:fourthDistribution}
        %     \end{subfigure}
        %     \vskip\baselineskip
        %     \begin{subfigure}{0.2\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_5.jpg}
        %         \caption{$\bar{x}_5 = 5.36, ba_5 = 8.14$.}
        %         \label{fig:fithDistribution}
        %     \end{subfigure}
        %     \caption{The five CVSS distribution generated to test the aggregation algorithm. Each one represents a different scenario to test the proposed aggregation algorithm. $\bar{x}$ represents the arithmetic mean of all the values, and $ab$, the result of the Bayesian addition proposed in this research work.}
        %     \label{fig:setOfDistributions}
        % \end{figure}


        % \begin{figure*}[!htb]
        %     \centering
        %     \begin{subfigure}{0.185\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_1.jpg}
        %         \caption{\centering$\bar{x}_1 = 5.11$\newline \centerline{$ba_1 = 8.04$}}
        %         \label{fig:firstDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.185\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_2.jpg}
        %         \caption{\centering$\bar{x}_2 = 7.09$\newline \centerline{$ba_2 = 8.59$}}
        %         \label{fig:secondDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.185\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_3.jpg}
        %         \caption[justification=centering]{\centering$\bar{x}_3 = 2.79$\newline \centerline{$ba_3 = 6.42$}}
        %         \label{fig:thirdDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.185\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_4.jpg}
        %         \caption{\centering$\bar{x}_4 = 5.14$\newline \centerline{$ba_4 = 8.05$}}
        %         \label{fig:fourthDistribution}
        %     \end{subfigure}
        %     \hfill
        %     \begin{subfigure}{0.185\textwidth}
        %         \includegraphics[width=\textwidth]{photo/distribution_5.jpg}
        %         \caption{\centering$\bar{x}_5 = 5.36$\newline \centerline{$ba_5 = 8.14$}}
        %         \label{fig:fithDistribution}
        %     \end{subfigure}
        %     \caption{The five CVSS distribution generated to test the aggregation algorithm. Each one represents a different scenario to test the proposed aggregation algorithm. $\bar{x}$ represents the arithmetic mean of all the values, and $ab$, the result of the Bayesian addition proposed in this research work.}
        %     \label{fig:setOfDistributions}
        % \end{figure*}


    \subsection{Corrected CVSS Values}
        After obtaining the final $\lambda$ factor for each CVSS, the new corrected CVSS values were calculated as indicated in line \textit{6} in Algorithm~\ref{alg:aggregation}. At this point, it is necessary to check for overflows: Every value higher than 10 was set to 10.


        \begin{table}[!htb]
            \centering
            \caption{Example of the data calculated for each dataset.}
            \label{tab:datasetSample}
            \resizebox{0.5\textwidth}{!}{%
            \begin{tabular}{@{}cccccccc@{}}
            \toprule
            \multicolumn{8}{c}{\textbf{DISTRIBUTION  \#1}}                                                                                                                        \\ \midrule
            \multicolumn{8}{c}{Nº of layers = 4}                                                                                                                                  \\ \midrule
            Interpolation: linear & \multicolumn{2}{c}{$y = mx * n$}   & \multicolumn{2}{c}{$m =-0.25$}            & \multicolumn{2}{c}{$n =1.25$}          &                     \\ \midrule
            \textbf{INITIAL CVSS} & \textbf{LAYER} & \textbf{DEEPNESS} & \textbf{FUNCTIONALITY} & \textbf{CONTEXT} & \textbf{EXPLOIT} & \textbf{SUMMARIZED} & \textbf{FINAL CVSS} \\ \midrule
            1                     & 2              & 0.75              & 1                      & 0                & 1                & 0                   & 0                   \\
            2                     & 1              & 1                 & 1                      & 1                & 1.25             & 1.25                & 2.5                 \\
            2                     & 1              & 1                 & 0                      & 1                & 1                & 0                   & 0                   \\
            4                     & 3              & 0.5               & 0                      & 1                & 1                & 0                   & 0                   \\
            $\vdots$              & $\vdots$       & $\vdots$          & $\vdots$               & $\vdots$         & $\vdots$         & $\vdots$            & $\vdots$            \\
            7                     & 2              & 0.75              & 1                      & 1                & 1                & 0.25                & 5.25                \\
            7                     & 4              & 0.25              & 0                      & 1                & 0                & 0                   & 0                   \\
            10                    & 4              & 0.25              & 1                      & 0                & 0                & 0                   & 0                   \\ \bottomrule
            \end{tabular}%
            }
        \end{table}

        
    \subsection{Average Factor Calculation}
        We decided to use the arithmetic mean for the sake of simplicity. In this stage, we computed the arithmetic mean of all the CVSS values to be aggregated ($64$ values for each distribution).


    \subsection{Calculation of the Aggregated Value}
        The final aggregation was implemented as shown in line \textit{11} in Algorithm~\ref{alg:aggregation}.


    \subsection{Results}
        Table~\ref{tab:aggregationResults} shows the obtained results for all five distributions.

        \begin{table}[!htb]
            \centering
            \caption{Results of the aggregation, using both the arithmetic and the harmonic means as average functions. For comparison, the arithmetic mean and the maximum value of each distribution are also shown.}
            \label{tab:aggregationResults}
            \resizebox{0.5\textwidth}{!}{%
            \begin{tabular}{@{}cccccc@{}}
                \toprule
                DISTRIBUTION  & $MEAN_{arith}$ & $MEAN_{armo}$ & MAGERIT & $BAYES_{arith}$ & $BAYES_{armo}$  \\ \hline
                \#1           & 5.11           & 4.49          & 10      & 8.04            & 7.77            \\
                \#2           & 7.09           & 4.73          & 10      & 8.59            & 7.89            \\
                \#3           & 2.79           & 1.41          & 10      & 6.42            & 2.92            \\
                \#4           & 5.14           & 1.31          & 10      & 8.05            & 2.35            \\
                \#5           & 5.36           & 2.51          & 10      & 8.14            & 4.82            \\ \bottomrule
            \end{tabular}%
            }
        \end{table}
        
        % This is specially reflected in the result of the aggregation of distribution 3 (Figure~\ref{fig:thirdDistribution}), that mainly contains low CVSS values: It is as critical to have a high CVSS that can be exploited, than it is to have several small CVSS scores that can be also exploited.

        Without the correction factors developed in this research, the formula proposed by MAGERIT would return a final result of $10$ for every distribution shown here. Nevertheless, taking into account features such as the exploitability of the vulnerabilities, the context of the SUT, or its functionalities, we can filter out the most important CVSS values to be aggregated. With such process, the total amount of CVSS values to be added is simplified. This also helps to simplify existing attack graphs and their analysis.

        % For Distribution 4 in Figure~\ref{fig:fourthDistribution}, the aggregated value is higher than the mean. In fact, the result is similar to the obtained for Distribution 1 in Figure~\ref{fig:firstDistribution}. This effect might be caused by two mechanisms:
        % \begin{itemize}
        %     \item \textbf{The generation of the correction factors:} They were generated randomly. This means that we cannot control which CVSS gets neglected. Using the arithmetic mean as the average correction factor might be also a cause of this phenomenon.
        %     \item \textbf{The extreme values in the dataset:} Low CVSS values contribute a minimal portion of the final result.
        % \end{itemize}

        Finally, it is worth highlighting that the only way to obtain a low value with the proposed algorithm is to have either 
        (1) a low number of low CVSS values to add, or 
        (2) a low value for the average correction factor.











    \begin{table}[!htb]
        \caption{XXXXXXXXXXXX XXXXXXXX XXX XX XXXXX XXXXXXXXXX XXXXX XXXX XXXX.}
        \label{tab:useCaseCVSS}
        \centering
        \begin{tabularx}{0.5\textwidth}{llXXXXXXXXX}
            \hline
            CVE & CVSS & AV & AC & PR & UI & S & C & I & A & E \\
            \hline
            CVE-2017-18269  & 9.8 & N & L & N & N & U & H & H & H & N \\
            CVE-2018-11236  & 9.8 & N & L & N & N & U & H & H & H & N \\
            CVE-2018-11237  & 7.8 & L & L & L & N & U & H & H & H & N \\
            CVE-2018-12886  & 8.1 & N & H & N & N & U & H & H & H & N \\
            CVE-2019-15847  & 7.5 & N & L & N & N & U & H & N & N & N \\
            \hline
            Arithmetic mean & 7.5 &   &   &   &   &   &   &   &   &   \\
            Harmonic mean   & 7.5 &   &   &   &   &   &   &   &   &   \\
            \hline
        \end{tabularx}%
    \end{table}
